Twist Decoding: Diverse Generators Guide Each Other

Many language generation models are now available for a wide range of generation tasks, including machine translation and summarization. Combining such diverse models may lead to further progress, but ensembling generation models is challenging during inference: conventional ensembling methods (e.g., shallow fusion) require that the models share vocabulary/tokenization schemes. We introduce Twist decoding, a simple and general text generation algorithm that benefits from diverse models at inference time. Our method does not assume the vocabulary, tokenization or even generation order is shared. Our extensive evaluations on machine translation and scientific paper summarization demonstrate that Twist decoding substantially outperforms each model decoded in isolation over various scenarios, including cases where domain-specific and general-purpose models are both available. Twist decoding also consistently outperforms the popular reranking heuristic where output candidates from one model are rescored by another. We hope that our work will encourage researchers and practitioners to examine generation models collectively, not just independently, and to seek out models with complementary strengths to the currently available models. Our code is available at https://github.com/jungokasai/twist_decoding.

==> text/experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}


T5 and GPT-3 (tasks?)
machine translation with two directions/different vocabs
constrained generation
baselines: single models, reranking


\begin{table}[t]
\addtolength{\tabcolsep}{-5.5pt}
\centering
\begin{subtable}[b]{.31\textwidth}
\centering
\begin{tabular}{@{} l cc m{0.0001em} cc m{0.0001em} cc @{}}
\toprule[.1em]

\textbf{WMT20} 
& \multicolumn{2}{c}{\textbf{EN$\rightarrow$DE}}
&& \multicolumn{2}{c}{\textbf{EN$\rightarrow$RU}}
\\
\cmidrule(lr){2-3}
\cmidrule(lr){5-6}
\textbf{Model} 
& COM & BLE
&& COM & BLE
\\

\midrule[.1em]

mBART
& 38.0
& 21.3 
&& 46.2
& 29.9
\\
Rerank 
& 39.4
& 21.5
&& 46.9 
& 30.1 

\\ 
Fusion & \\ 

\bottomrule[.1em]
\end{tabular}
\caption{Fusion between a large, monolingual language model and a transformer machine translation model.} 
\end{subtable}%
\hfill
\begin{subtable}[b]{.31\textwidth}
\centering
\begin{tabular}{@{} l cc m{0.001em} cc m{0.001em} cc @{}}
\toprule[.1em]

& \multicolumn{2}{c}{\textbf{COVID}}
&& \multicolumn{2}{c}{\textbf{Subtitles?}}
\\
\cmidrule(lr){2-3}
\cmidrule(lr){5-6}
\textbf{Model} 
& COM & BLE
&& COM & BLE
\\

\midrule[.1em]
Expert
&  
& 37.1 
\\


mBART
& 10.0 
& 10.0
&& 10.0
& 10.0
\\
Rerank & \\ 
Fusion & \\ 

\bottomrule[.1em]
\end{tabular}
\caption{COVID19: Korean$\rightarrow$English COVID19 KCDC data \citep{berard-etal-2020-multilingual}. Others are the German$\rightarrow$English data from \citet{}.} 
\end{subtable}%
\hfill
\begin{subtable}[b]{.31\textwidth}
\centering
\begin{tabular}{@{} l cc m{0.0001em} cc  @{}}
\toprule[.1em]

\textbf{WMT20}
& \multicolumn{2}{c}{\textbf{ZH$\rightarrow$EN}}
&& \multicolumn{2}{c}{\textbf{EN$\rightarrow$DE}}\\
\cmidrule(lr){2-3}
\cmidrule(lr){5-6}
\textbf{Model}
& \textsc{COM} & \textsc{BLE}
&& \textsc{COM} & \textsc{BLE}
\\

\midrule[.1em]
L2R & 40.8 & 35.5 & & 42.9 & 45.5\\
R2L & 40.4 & 35.0 & & 43.3 &  44.9\\
Rerank & 41.4& 36.1 & &43.7 & 46.0  \\
Fusion & \textbf{43.4} & \textbf{37.1} &&\textbf{45.9} & \textbf{46.8}\\
\bottomrule[.1em]
\end{tabular}
\caption{
L2R: left-to-right. R2L: right-to-left. ZH: Chinese. DE: German.
} 
\end{subtable}%

\caption{Machine translation results over various settings. (a) language model fusion. (b) domain adaptation. (c) combining left-to-right and right-to-left models. COM and BLE denote the COMET \cite{comet-wmt} and BLEU \citet{Papineni2001BleuAM} metrics.
COMET uses crosslingual contextual representations from XLM-RoBERTa \citep{conneau-etal-2020-unsupervised} and has shown to have significantly higher correlation with human judgment than ngram-based, conventional metrics, such as BLEU \citep{mathur-etal-2020-results,billboard}.}
\end{table}


\subsection{Experimental Setup and Baselines}

\subsection{Machine Translation}
\paragraph{Different Domains}
\paragraph{Left-to-Right and Right-to-Left}
We experiment with two language pairs from the WMT 2020 news translation task \cite{barrault-etal-2020-findings}: Chinese$\rightarrow$English (\textbf{WMT20 ZH-EN}) and English$\rightarrow$German (\textbf{WMT20 EN-DE}).
We use outputs from all submitted translation systems.\footnote{\url{https://www.statmt.org/wmt20/translation-task.html}.}
These two language pairs have expert, rubric-based scores (MQM) from \citet{freitag2021experts} for a subset of 10 submitted systems, including the top-performing systems and human translations.
Each output sentence is evaluated by three professional translators.
Following \citet{freitag2021experts}, the three scores are averaged to get an instance-level score.

We use all human translations available as a reference set for reference-based metrics.
Concretely, every test instance in WMT20 ZH-EN has two translations provided by different human translation services: Human-A and Human-B \cite{barrault-etal-2020-findings}.
In addition to Human-A and Human-B, WMT20 EN-DE provides a translation that is created by linguists who are asked to paraphrase Human-A and Human-B as much as possible (Human-P, \citealp{freitag-bleu-paraphrase-references-2020}).
These paraphrased translations are shown to increase correlations with human judgments by mitigating the \textit{translationese effect} and diversifying the reference when the generation quality is measured by reference-based metrics \cite{freitag-bleu-paraphrase-references-2020}.

\subsection{Grammatical Error Correction}

\subsection{Abductive Reasoning?}

\subsection{Baselines}
\paragraph{Reranking}



Along with all submitted generators in WMT20 ZH-EN and WMT20 EN-DE, we train three transformer baselines with the \texttt{fairseq} library \cite{ott-etal-2019-fairseq} and place them in our \bilboards: \textbf{transformer-base}, \textbf{transformer-large}, and \textbf{transformer-large-ensemble} with similar hyperparameters (e.g., 6-layer encoder and decoder) to the ones trained on WMT16 EN-DE data in \citet{Vaswani2017AttentionIA}.\footnote{We make our preprocessed data and the baseline models available at \url{https://github.com/jungokasai/billboard}.}
These baselines allow researchers to compare their translation models without resource-intensive techniques such as backtranslation \cite{sennrich-etal-2016-improving}, model ensembling, and deep encoders \cite{deepshallow}.
These techniques are all used in top-performing systems of WMT20 \cite{wu-etal-2020-volctrans, kiyono-etal-2020-tohoku} but might be infeasible in many research settings.
See Appendix \ref{appendix:generators} for a list of all hyperparameters for the baselines.



\paragraph{Summarization}
We use the CNN/DailyMail corpus (\textbf{CNNDM}, \citealp{cnndaily, nallapati-etal-2016-abstractive}).
We use the standard train/dev./test split and 24 models from \citet{fabbri2021summeval}.
100 test articles are annotated with 10 summaries written by humans \cite{kryscinski-etal-2019-neural}.
For those 100 articles, rubric-based, expert evaluations for 18 generators, including human-written highlights, are provided by \citet{fabbri2021summeval}.\footnote{Some of the model outputs are lowercased and/or tokenized. In these cases, we apply the NLTK detokenizer \cite{nltk} and/or Stanford CoreNLP truecaser \cite{manning-EtAl:2014:P14-5}. We encourage, however, future model developers to provide clean, untokenized output to improve the reproducibility and transparency of evaluation results \cite{post-2018-call, kasai2021thumb}.}
Each output summary is evaluated by three experts along four dimensions: \textit{coherence} (collective quality of all summary sentences), \textit{consistency} (factual alignment with the article, penalizing for hallucinations), \textit{fluency} (quality of the individual sentences), and \textit{relevance} (selection of important content).
An instance-level score is computed by averaging scores over all these categories and the three experts.
Note that this aggregation method can be modified, depending on the downstream of interest \cite{kasai2021thumb}.
All 10 human-written summaries are used as the reference set for reference-based metrics.\footnote{Prior work used a concatenation of author-written highlights as a reference, but here we do not add it to the reference set. This is because these highlights are sometimes noisy (e.g., containing urls) or lack coherence because they are concatenations of separate bullet points \cite{fabbri2021summeval}.}


==> text/intro_old.tex <==
\begin{figure}[t!]
\centering
    \includegraphics[width=0.48\textwidth]{figs/twist_decoding.pdf}
\caption{\twist decoding of two generation models, $f$ and $g$, that does not assume a shared vocabulary, tokenization, or generation order.
Beam search is first applied to $f$ to generate $\vy$, followed by output mapping to $\widetilde{\vy}$ (e.g., $f$'s detokenization and $g$'s tokenization).
$g$ is then decoded with beam search augmented with distances from the set of previously-generated outputs (here only one sequence $\widetilde{\mathbf{y}}$ is shown): \textcolor{dblue}{$d(\vz_{\leq n}, \widetilde{\vy}_{\leq n})$}.
Subsequently, $f$ is similarly decoded with $g$'s guidance.
Here we show one iteration that already achieves substantial improvements (\S\ref{sec:analysis}), but additional iterations can be made.
}
\label{fig:twist_decoding}
\vspace{-0.0cm}
\end{figure}
\section{Introduction}
Natural language generation has now become important building blocks for many applications, such as machine translation, summarization, and question answering \interalia{ng-etal-2019-facebook,lewis-etal-2020-bart,T5,gpt3,asai2021cora}.
Language generation involves \textit{decoding}, an inference procedure that generates high-scoring (or high-probability) text under a generation model.
Researchers have recently explored and advanced models for generation in various aspects, including model architecture \cite{Bahdanau2014NeuralMT,Vaswani2017AttentionIA}, domain adaptation \cite{chu-wang-2018-survey,bapna-firat-2019-simple}, prompting \cite{gpt3}, and even generation order \cite{Gu2017NonAutoregressiveNM}.
These diverse generation models and their corresponding pipelines (e.g., pre/postprocessing such as (de)tokenization and text normalization) are typically developed independently by researchers or practitioners, and the models are decoded in \textit{isolation}.
In this work, we explore a contrasting question: can we blend strengths of diverse generation models to produce higher-quality text than each used alone without any additional training?


We introduce a new inference algorithm, \twist decoding (Fig.\ \ref{fig:twist_decoding}), that enables diverse generators to guide each other.
\twist decoding does not assume the vocabulary, (de)tokenization, and even generation order are shared between models.
This contrasts with the widely-used ensembling or shallow-fusion technique \interalia{Sutskever2014SequenceTS,shallow-deep-fusion,firat-etal-2016-zero} that adds scores at every step of beam search.
Our method decodes a model by standard beam search, but the scores at every step are augmented with a simple function that measures the distance from outputs of the other model.
We run this procedure on each generation model in turn, so that both can benefit from each other.
This modification in beam search can be implemented with a change in a \greenbox{single line of code} and requires no change to the trained models themselves.

We present extensive experiments on machine translation and scientific paper summarization and show that \twist decoding can improve performance over each model decoded alone in several scenarios: combining 1) generic and domain-specific models, 2) left-to-right and right-to-left generation models, and 3) models that take different parts of input documents. 
As language generation models continue to scale up, training or finetuing becomes prohibitively expensive computationally (and thus financially and environmentally; \citealp{strubell-etal-2019-energy,greenai}).
\twist decoding therefore have benefits of avoiding such costly procedures.
Further, our results show consistent performance gains from combining generic and domain-specific translation models over a wide range of domains, including medical and legal translation; applications in these domains need particularly high accuracy, and \twist decoding is a desirable alternative to standard beam search on a single model.
Interestingly, we find that \twist decoding between generic and domain models is effective even when parallel data from the domain are scarce and the domain model yields poor performance by itself, suggesting complementary
strengths of diverse generators (\S\ref{sec:low-resource}).

\twist decoding can be seen as a generalization of reranking heuristics that have proven effective in syntactic parsing \cite{shen-joshi-2003-svm,collins-koo-2005-discriminative}, speech recognition \cite{collins-etal-2005-discriminative}, and machine translation \cite{shen-etal-2004-discriminative,och-etal-2004-smorgasbord}: one model generates candidate sequences, followed by rescoring from another model.
We present extensive comparisons with reranking baselines and demonstrate that \twist decoding outperforms reranking consistently.
We also observe that since the encoder computations on two models can be parallelized, the inference time required for \twist decoding is much shorter than the sum of the two models, resulting only in a 50-\% increase, relative to decoding of a single model (\S\ref{sec:analysis}).
\twist decoding is therefore a viable alternative to standard beam search on a single model and the widespread reranking heuristic.

==> text/method_old.tex <==
\begin{figure}[t!]
\algrenewcommand{\algorithmiccomment}[1]{\hskip1em\# \footnotesize#1 \small}
\begin{algorithm}[H]
\small
$M$: maximum length.\\
$\vocab_g$: vocabulary of $g$. \quad $g(\cdot)$: scoring function.\\
$\mathcal{Y}^{(t-1)}$: set of output sequences from $f$ \quad $\mathcal{Z}^{(t)}$: new outputs\\
$B_n$: beam of continuing sequences\\
$H$: expanded hypotheses before beam selection\\
\greenbox{$d(\cdot,\cdot)$}: distance between partial sequences\\
\greenbox{$\lambda_f$}: scalar coefficient for the distance
\begin{algorithmic}[1]
\small
\State $\widetilde{\mathcal{Y}}^{(t-1)} =  \left\{ \widetilde{\vy} = \mapoutput(\vy) | \vy \in \mathcal{Y}^{(t-1)} \right\}$ \label{line:map_output}
\State $B_{0} \gets \{ \bos \}$, $\mathcal{Z}^{(t)}  \gets \varnothing $ 
\For{ $n \in \{ 1, \dots, M\!-\! 1 \}$ }
    \State $H \gets \varnothing$
    \For{$ \vz \in B_{n-1}$} \algorithmiccomment{Expansion.}
    \For{$z \in \vocab_g$}
        \State $s \gets g(\rvz \circ z)$\colorbox{green!25}{$- \lambda_f \min_{\widetilde{\vy} \in \widetilde{\mathcal{Y}}^{(t-1)}} d \left(\rvz \circ z,  \widetilde{\rvy}_{\leq n}\right)$}  \label{line:bs-score-eval}
        \State $H.\mathrm{add}( \langle s, \vz \circ z \rangle)$
    \EndFor
    \EndFor
 \State $B_n \gets \varnothing$
     \While{$ |B_n| < k$}  \algorithmiccomment{Find $\topk$ w/o $\eos$ from $H$.}
    \small \State $ \langle s, \vz \rangle \gets H.\mathrm{max}()$  
\small
     \If{\ $\vz.\mathrm{last}() = \eos$}
        \State $\mathcal{Z}^{(t)}.\mathrm{add}(\vz)$    \algorithmiccomment{Finished hypotheses.}\label{line:fcfs_f}
    \small \Else{\ $B_n.\mathrm{add}{(\vz)}$}
     \EndIf
    \small  \State $H.\mathrm{remove}(\langle s, \vz \rangle)$
\EndWhile
\EndFor
\State \Return $\mathcal{Z}^{(t)}$

\end{algorithmic}
\caption*{\small \textbf{\twist Decoding}\\$g$ generates $\vz$ with guidance from $f$ at iteration $t$}
\end{algorithm}
\caption{
\twist decoding when $g$ is guided by $f$.
Swap $f$ and $g$ and $\vy$ and $\vz$ to obtain $\mathcal{Y}^{(t)}$.
$\mapoutput$ converts outputs from $f$ to $g$; e.g., $f$'s detokenization followed by $g$'s tokenization. It would also include sequence reversal if $f$ or $g$ is a right-to-left model.
The \greenbox{highlighted line} is the \textit{only} modification that \twist decoding introduces to standard beam search.
The input sequence to $g$ is omitted.
See also \citet{kasai2022beampatience} for the stopping criterion and implementation details.
}
\label{alg:twist}
\end{figure}
\section{\alt Decoding}
\label{sec:twist_decoding}
We propose \twist decoding, a general decoding algorithm that generates text from diverse models without assumptions of a shared vocabulary, tokenization, or generation order.
At the core of the algorithm is a simple modification in standard beam search (\greenbox{highlighted} in Fig.\ \ref{alg:twist}); we incorporate into a scoring function the distance from outputs that are previously generated by another model.

\subsection{Initial Decoding}
Let us assume that we have two generation models: $f$ and $g$.\footnote{The algorithm can be readily extended to three or more generators. We also abuse $f$ or $g$ to mean both the generator and its scoring function.}
Both $f$ and $g$ assign scores to output sequences.\footnote{They typically assign $log$ probabilities, but it is not necessary to assume the scores form a valid probability distribution.}
$f$ is, for instance, a domain-specific translation model and $g$ a generic translation model.  
$f$ and $g$ perform their own pre/postprocessing (e.g., (de)tokenization) and factorization (e.g., left-to-right or right-to-left factorization).
Here we suppress for brevity the input condition (e.g., machine translation input from the original language).
 Standard beam search with beam size $k$ (\textit{first come, first served} implementation; \citealp{kasai2022beampatience}) is first applied to $f$ to produce a set of $k$ output sequences: $\mathcal{Y}^{(0)}$.
 This approximately solves $\topk_{\vy} f\left( \vy \right)$ by pruned breadth-first search, and often returns higher-quality outputs than the exact search counterpart \cite{stahlberg-byrne-2019-nmt,meister-etal-2020-beam}.



\subsection{Mutually-Guided Decoding}
\label{sec:mutual_guidance}
Once $\mathcal{Y}^{(0)}$ is obtained, we proceed with decoding generators with mutual guidance (Fig.\ \ref{alg:twist}; $t \geq 1$)
\paragraph{Output Sequence Mapping}
The commonly-used technique of ensembling \cite{Sutskever2014SequenceTS} or shallow fusion \cite{shallow-deep-fusion,stahlberg-etal-2018-simple} adds scores from $f$ and $g$ at every step and executes the same search algorithm to approximately solve $\topk_{\vy} f(\vy) + g(\vy)$.
This method thus necessitates a shared vocabulary, tokenization, and generation order \cite{imamura-sumita-2017-ensemble}.
We depart from this assumption and first map the candidates in $\mathcal{Y}^{(t-1)}$ to output sequences for $g$: $\widetilde{\mathcal{Y}}^{(t-1)}$ (Line \ref{line:map_output} in Fig.\ \ref{alg:twist}).
This mapping ($\mapoutput$) typically involves deterministic operations of $f$'s detokenization followed by $g$'s tokenization.
Sequence reversal is also performed if $f$ and $g$ generate in the opposite order.
For instance, $\vy\!=$\textit{John does n't like Mary} can be mapped to $\widetilde{\vy}\!=$\textit{Jo@ doesn't like Mar@ y}, where @ denotes subword separation in byte pair encoding \cite{sennrich-etal-2016-neural} that $g$ uses, but not $f$.

\paragraph{Decoding with Distance Terms}
We then decode $g$ with guidance from $\widetilde{\mathcal{Y}}^{(t-1)}$.
Specifically, we perform beam search with a simple modification in scoring (\setlength{\fboxsep}{1.0pt}{\colorbox{green!25}{Line \ref{line:map_output}}}).
In this work, we use a simple distance measure that adds binary distances at all positions (i.e., Hamming distance):
\begin{align*}
d \left ( \vz_{\leq n}, \widetilde{\vy}_{\leq n} \right) =  \sum_{i \leq n} \diff \left(z_{i}, \widetilde{y}_i \right),\\
\text{where \quad } \diff(z_i, \widetilde{y}_i) = 1- \mathbbm{1} \left\{z_{i} = \widetilde{y}_i \right\} 
\end{align*}
We also explored using  between (sub)word embeddings from the model: $\diff(z_i, \widetilde{y}_i) \!=\! \lVert e (z_i) - e (\widetilde{y}_i) \rVert_2$, but this did not bring improvements (\S\ref{sec:analysis}).
Note also that when $i$ exceeds the length of $\widetilde{y}$, we assume $\widetilde{y}_i = \eos$.
The overall distance term is then 
\begin{align*}
\min_{\widetilde{\vy} \in \mathcal{Y}^{(t-1)}} d \left ( \vz_{\leq n}, \widetilde{\vy}_{\leq n} \right)
\end{align*}
Here we minimize over the output sequences to compute the distance to the closest candidate.
These candidates from $\mathcal{Y}^{(t-1)}$ can be equally good outputs but differ only by one word; in such cases, this minimization operation avoids overestimation of the distances.
The new score at step $n$ in beam search is now computed by:
\begin{align*}
 g(\vz_{\leq n}) - \lambda_f \min_{\widetilde{\vy} \in \widetilde{\mathcal{Y}}^{(t-1)}} d \left(\vz_{\leq n},  \widetilde{\rvy}_{\leq n}\right),
\end{align*}
where $\lambda_f$ is a scalar coefficient for the distance term that controls the importance of $f$ relative to $g$.
We tune $\lambda_f \in \{0.1, 0.3, 1.0, 3.0\}$ during development.
After this beam search, we obtain a new candidate set, $\mathcal{Z}^{(t)}$.
We then run the same beam search (Fig.\ \ref{alg:twist}) with the roles of $f$, $\mathcal{Y}$ and $g$, $\mathcal{Z}$ swapped.
Namely, we decode $f$ with distance terms from $\mathcal{Z}^{(t)}$ at each step of beam search:
\begin{align*}
 f(\vy_{\leq n}) - \lambda_g \min_{\widetilde{\vz} \in \widetilde{\mathcal{Z}}^{(t)}} d \left(\vy_{\leq n},  \widetilde{\vz}_{\leq n}\right)
\end{align*}
Finally, the highest-scoring sequence from $\mathcal{Y}^{(t)}$ is outputted.
This process of mutually-guided decoding can be repeated multiple times.
We observe, however, that one iteration ($t=1$) suffices to bring performance gains (\S\ref{sec:analysis}).
We also present detailed sensitivity analysis over varying $\lambda_f$ and $\lambda_g$ and find that \twist decoding is particularly effective when $\lambda_g > \lambda_f$ (i.e., initial exploration by $g$ is encouraged with relatively little guidance from $f$'s original outputs; see Section \S\ref{sec:analysis}).

\begin{table*}[t]
\addtolength{\tabcolsep}{-1.0pt}
\centering
\small
\begin{tabular}{@{} lcc   m{0.01em}  cc   m{0.01em}   cc m{0.01em}  cc m{0.01em}   cc @{}}
\toprule[.1em]

 \multicolumn{3}{c}{\textbf{German$\rightarrow$English}}
&& \multicolumn{2}{c}{\textbf{Medicine}}
&& \multicolumn{2}{c}{\textbf{Law}}
&& \multicolumn{2}{c}{\textbf{Koran}}
&& \multicolumn{2}{c}{\textbf{Subtitles}}
\\
\cmidrule(lr){5-6}
\cmidrule(lr){8-9}
\cmidrule(lr){11-12}
\cmidrule(lr){14-15}
\textbf{Method} 
& $f$ 
& $g$
&& COMET & BLEU
&& COMET & BLEU
&& COMET & BLEU
&& COMET & BLEU
\\

\midrule[.1em]

Isolation
& Generic
& --
&& 44.5    
& 41.2 
&& 30.6 
&  34.8 
&&  14.4
& 16.6 
&& 34.4 
&31.3
\\
Isolation
& Domain
& --
&& 80.7
& 48.3 
&& 60.7 
&  40.9
&&  8.7
& 17.0
&& 32.3
& 29.0 
\\


\midrule[.05em]


Rerank
& Generic
& Domain
&& 59.6
& 43.5 
&& 56.4
& 36.1
&& 14.7 
& 17.0 
&& 40.3 
&  \textbf{32.3}

\\ 

\rowcolor[gray]{.93}
\textbf{\alt}
& Generic
& Domain
&& 71.6 
& 47.5
&&  61.4
& 40.2 
&& \textbf{16.5}
&  18.5
&& \textbf{41.0}
&  32.2


\\
\multicolumn{3}{l}{$\Delta$ (\textbf{\alt}$-$ Rerank)}
&& \textblue{$+12.0$}
& \textblue{$+4.0$}
&& \textblue{$+5.0$}
& \textblue{$+4.1$}
&& \textblue{$+1.8$}
&  \textblue{$+1.5$}
&& \textblue{$+0.7$}
& \textred{$-0.1$}

\\
 \cdashlinelr{1-15}

Rerank
& Domain
& Generic
&& 75.8
& 48.7
&& 59.9
& 40.8
&& 12.3
&  18.1
&& 36.5 
& 30.3 
\\ 

\rowcolor[gray]{.93}
\textbf{\alt}
& Domain
& Generic
&& \textbf{81.6}
& \textbf{50.1} 
&& \textbf{61.6} 
& \textbf{41.3}
&& 15.3
& \textbf{18.7} 
&&  37.3
&  31.0
\\


\multicolumn{3}{l}{$\Delta$ (\textbf{\alt}$-$ Rerank)}
&& \textblue{$+5.8$}
& \textblue{$+1.4$}
&& \textblue{$+1.7$}
& \textblue{$+0.5$}
&& \textblue{$+3.0$}
&  \textblue{$+0.6$}
&& \textblue{$+0.8$}
& \textblue{$+0.7$}

\\


\bottomrule[.1em]
\end{tabular}
\caption{
Combination of generic and domain-specific translation models.
The generic model is the top-performing translation model in WMT19 \citep{ng-etal-2019-facebook} that is trained on a collection of parallel corpora, such as the Europarl and the UN corpora.
Two settings are considered for each of the reranking base and our \twist decoding: $f$ is the generic model and $g$ is the domain-specific model or the reverse.
The best scores are in \textbf{bold}. COMET \cite{rei-etal-2020-comet,comet-wmt} uses crosslingual contextual representations \cite{conneau-etal-2020-unsupervised} and achieves significantly higher correlation with expert human judgment than BLEU \cite{Papineni2001BleuAM} and other alternative metrics \cite{billboard,kasai2021thumb}.
}
\label{tab:domain_results}
\end{table*}%

\paragraph{Reranking Heuristic as a Special Case}
Notice that as $\lambda_{f} \rightarrow \infty$, $g$'s generation falls back to a reranking heuristic: top $k$ sequences from the initial $f$ decoding are reranked according to $g$.
This reranking heuristic has proven successful in a wide range of sequence generation tasks, including machine translation \cite{shen-etal-2004-discriminative}, syntactic parsing \cite{collins-koo-2005-discriminative}, and speech recognition \cite{collins-etal-2005-discriminative}.
Reranking is performed in many strong machine translation systems to use a right-to-left model to improve a left-to-right model; e.g., top-performing systems in recent WMT competitions \cite{ng-etal-2019-facebook,kiyono-etal-2020-tohoku,wang-etal-2021-tencent,akhbardeh-etal-2021-findings}.
In our experiments, we extensively compare performances of \twist decoding and reranking and demonstrate that the former consistently outperforms the latter.
